When Algorithms for Maximal Independent Set and Maximal Matching Run in Sublinear-Time

Maximal independent set (MIS), maximal matching (MM), and $(\Delta+1)$-coloring in graphs of maximum degree $\Delta$ are among the most prominent algorithmic graph theory problems. They are all solvable by a simple linear-time greedy algorithm and up until very recently this constituted the state-of-the-art. In SODA 2019, Assadi, Chen, and Khanna gave a randomized algorithm for $(\Delta+1)$-coloring that runs in $\widetilde{O}(n\sqrt{n})$ time, which even for moderately dense graphs is sublinear in the input size. The work of Assadi et al. however contained a spoiler for MIS and MM: neither problems provably admits a sublinear-time algorithm in general graphs. In this work, we dig deeper into the possibility of achieving sublinear-time algorithms for MIS and MM. The neighborhood independence number of a graph $G$, denoted by $\beta(G)$, is the size of the largest independent set in the neighborhood of any vertex. We identify $\beta(G)$ as the ``right'' parameter to measure the runtime of MIS and MM algorithms: Although graphs of bounded neighborhood independence may be very dense (clique is one example), we prove that carefully chosen variants of greedy algorithms for MIS and MM run in $O(n\beta(G))$ and $O(n\log{n}\cdot\beta(G))$ time respectively on any $n$-vertex graph $G$. We complement this positive result by observing that a simple extension of the lower bound of Assadi et.al. implies that $\Omega(n\beta(G))$ time is also necessary for any algorithm to either problem for all values of $\beta(G)$ from $1$ to $\Theta(n)$. We note that our algorithm for MIS is deterministic while for MM we use randomization which we prove is unavoidable: any deterministic algorithm for MM requires $\Omega(n^2)$ time even for $\beta(G) = 2$.

==> app-mm-lower.tex <==

\section{A Lower Bound for Deterministic Maximal Matching}\label{app:mm-lower}

We prove Theorem~\ref{thm:mm-lower} in this appendix, restated below for connivence of the reader. 

\begin{theorem*}
	Any deterministic algorithm that finds a maximal matching in every given graph $G$ with neighborhood independence $\beta(G) = 2$ (known to the algorithm) presented in the adjacency array representation requires $\Omega(n^2)$ time.
\end{theorem*}

For every integer $n=8k$ for $k \in \IN$, we define $\FG_n$ as the family of all graphs obtained by removing a perfect matching from a clique $K_n$ on $n$ vertices.
For a graph $G$ in $\FG_n$ we refer to the removed perfect matching of size $5k$ as the \emph{non-edge matching} of $G$ and denote it by $\bM(G)$. Clearly, every graph
in $\FG_n$ has neighborhood independence $\beta(G) = 2$. Moreover, any MM in $G$ can have at most $2$ unmatched vertices.


Let $\alg$ be a deterministic algorithm for computing an MM on every graph in $\FG_n$. We prove Theorem~\ref{thm:mm-lower} by analyzing a game between $\alg$ and an adaptive adversary that
answers the probes of $\alg$ to the adjacency array of the graph. In particular, whenever $\alg$ probes a \emph{new} entry of the adjacency array for some vertex $v \in V$, we can think of $\alg$ making a \emph{query} $Q(v)$ to
the adversary, and the adversary outputs a vertex $v$ that had not been so far revealed in the neighborhood of $u$ (as degree of all vertices in $G$ is exactly $n-1$, $\alg$ knows the degree of all vertices and we assume it never queries a vertex $u$ more than
$n-1$ times).

We now show that there is a strategy for the adversary to answer the queries of $\alg$ in a way that ensures $\alg$ needs to make $\Omega(n^2)$ queries before it can output an MM of the graph.


\paragraph{Adversary's Strategy:} The adversary picks an arbitrary set of $2k$ vertices $D$ referred to as \emph{dummy} vertices. We refer to remaining vertices as \emph{core} vertices and denote them by $C:= V \setminus D$.
The adversary also fixes a non-edge matching of size $k$ between vertices in $D$, denoted by $\bM_D$.
The non-edge matching of $G$ consists of $\bM_D$ and a non-edge matching of size $4k$ between vertices in $C$, denoted by $\bM_C$, which unlike $\bM_D$ is constructed adaptively by the adversary.
We assume $\alg$ knows the partitioning of $V$ into $D$ and $C$, as well as the non-edge matching $\bM_D$. Hence, the only missing information to $\alg$ is identity of $\bM_C$.

To answer a query $Q(u)$ for a dummy vertex $u \in D$, the adversary simply returns any arbitrary vertex in $V$ (not returned so far as an answer to $Q(u)$) except for the pair of $u$ in $\bM_D$ which cannot be neighbor to $u$.
To answer the queries $Q(w)$ for core vertices $w \in C$, the adversary maintains a partitioning of $C$ into $\Cused$ and $\Cfree$. Initially all core vertices belong to $\Cfree$ and hence $\Cused$ is empty.
Throughout we only move vertices from $\Cfree$ to $\Cused$. The adversary also maintains a counter for every vertex in $\Cfree$ on how many times they have been queried so far.
Whenever a vertex $w \in \Cfree$ is queried, as long as this vertex has been queried at most $k$ times, the adversary returns an arbitrary dummy vertex $u$ from $D$ as the answer to $Q(w)$ (which is possible because of size of $D$ is $k$).
Once a vertex $w \in \Cfree$ is queried for its $(k+1)$-th time, we pick another vertex $w'$ from $\Cfree$ also, add the pair $(w,w')$ to the non-edge matching $\bM_C$ and move both $w$ and $w'$ to $\Cused$,
and then answer $Q(w)$ for the case $w \in \Cused$ as described below.

Recall that for any vertex $w \in \Cused$, by construction, there is another fixed vertex $w'$ in $\Cused$ (joined at the same time with $w$) where $(w,w') \in \bM_C$. For any query for $w \in \Cused$, the adversary answers $Q(w)$ by returning an arbitrary vertex
from $C \setminus \set{w'}$. This concludes the description of the strategy of the adversary.

\medskip
We have the following basic claim regarding the correctness of the adversary's strategy. %The proof is straightforward.

\begin{claim}\label{clm:adversary-correct}
	The answers returned by the adversary for any sequence of queries are always consistent with at least one graph $G$ in $\FG_n$.
\end{claim}
\begin{proof}
	We can append the current sequence of queries by the sequence that ensures all vertices are queried  $n-1$ times. Thus,
	the adversary would eventually construct the whole non-edge matching $\bM_C$ also. There exists a unique graph $G$ in $\FG_n$ where $\bM(G) = \bM_D \cup \bM_C$, hence proving the claim (note that before appending the sequence,
	there can be more than one graph consistent with the original sequence).
\end{proof}

We now prove the following lemma which is the key step in the proof of Theorem~\ref{thm:mm-lower}.
\begin{lemma}\label{lem:mm-contradiction}
	Suppose $\alg$ makes at most $k^2$ queries to the adversary and outputs a matching $M$ using only these queries. Then, there exists some graph $G$ in $\FG_n$ where $G$ is consistent with the answers returned by the adversary to $\alg$
	and $\bM(G) \cap M \neq \emptyset$.
\end{lemma}
\begin{proof}
	Since $\alg$ makes at most $k^2$ queries, there can only be $2k$ vertices in $\Cused$ by the time the algorithm finishes its queries (as each pair of vertices in $\Cused$ consumed $k$ queries).
	Consider the maximal matching $M$. There are at most $2k$ edges of $M$ that are incident on $\Cused$ and $k$ more edges incident on $D$. This implies that at most $3k$ vertices in $\Cfree$ are matched to vertices
	outside $\Cfree$. As $\card{\Cfree} \geq 5k$, it means that there are at least $2k$ vertices in $\Cfree$ that are not matched by $M$ to vertices outside $\Cfree$. However, as $M$ is maximal, and since $G$ is in $\FG_n$,
	there should be at least $k-1$ edges in $M$ between these vertices in $\Cfree$. As the adversary has not committed to the non-edge matching $\bM_C$ entirely at this point and this non-edge matching pairs vertices in $\Cfree$ to each other,
	the adversary can simply let $\bM_C$ contains $M$ and still obtain a graph $G$ in $\FG_n$. For this graph, $\bM(G) \cap M \neq \emptyset$, finalizing the proof.
\end{proof}

Theorem~\ref{thm:mm-lower} now follows immediately from Lemma~\ref{lem:mm-contradiction}, as it state that unless the algorithm makes $\Omega(n^2)$ queries, there always exists at least one graph in $\FG_n$ for which the output matching of the algorithm is
not feasible. As graphs in $\FG_n$ all have $\beta(G) = 2$, we obtain the final result.


